Towards Transferable Multi-modal Perception Representation Learning for Autonomy: NeRF-Supervised Masked AutoEncoder

This work proposes a unified self-supervised pre-training framework for transferable multi-modal perception representation learning via masked multi-modal reconstruction in Neural Radiance Field (NeRF), namely NeRF-Supervised Masked AutoEncoder (NS-MAE). Specifically, conditioned on certain view directions and locations, multi-modal embeddings extracted from corrupted multi-modal input signals, i.e., Lidar point clouds and images, are rendered into projected multi-modal feature maps via neural rendering. Then, original multi-modal signals serve as reconstruction targets for the rendered multi-modal feature maps to enable self-supervised representation learning. Extensive experiments show that the representation learned via NS-MAE shows promising transferability for diverse multi-modal and single-modal (camera-only and Lidar-only) perception models on diverse 3D perception downstream tasks (3D object detection and BEV map segmentation) with diverse amounts of fine-tuning labeled data. Moreover, we empirically find that NS-MAE enjoys the synergy of both the mechanism of masked autoencoder and neural radiance field. We hope this study can inspire exploration of more general multi-modal representation learning for autonomous agents.

==> figs/fig_teaser.tex <==



==> figs/overview.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{images/overview.pdf}
  \caption{Overview of the approach. The backbone to pre-train produces latent vectors for each input point. At pre-training time, the latent vector is fed into a volumetric occupancy head that classifies query points as full or empty. At semantic training or test time, the same latent vectors are fed into a semantic head, e.g., for semantic segmentation or object detection.}
  \label{fig:overview}
\end{figure*}

==> tables/ablation_single_stage_ft.tex <==
\renewcommand{\arraystretch}{0.3}
\begin{table}[t]
%\small
\resizebox{0.48\textwidth}{!}
	{
        \setlength{\tabcolsep}{2pt}
	\centering
	\begin{tabular}{l|c|cc|cc}
          \toprule
        \multirow{6}{*}{Method}  & \multirow{2}{*}{Pre-training}  &\multicolumn{2}{c|}{{Image: $128\times352$}}  &\multicolumn{2}{c}{{Image: $256\times704$}}     \\
         & \multirow{2}{*}{Type} &\multicolumn{2}{c|}{{\#Lidar Sweep: 1}}  &\multicolumn{2}{c}{{\#Lidar Sweep: 9}}     \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} 
      %   \midrule
         & & \quad mAP & NDS & \quad mAP & NDS  
         \\  \midrule
          BEVFusion& No   & \quad{50.5} &{53.3} &\quad {60.8} &{64.1}  \\ 
          + iNet  &Fully-supervised  &\quad{51.4} &{54.1}      &\quad{62.8} &{65.3}     
         \\  
        + \name  & Self-supervised  & \quad\textbf{{51.5}} &\textbf{54.7}      & \quad\textbf{{63.0}} &\textbf{65.5} 
         \\          

        \bottomrule
	\end{tabular}
       }
        %\vspace{1mm}
	\caption{\textbf{Comparison to supervised pre-training for Multi-modal Perception} model (BEVFusion~\cite{liu2022bevfusion}) on the 3D object detection task on \nus{} \cite{Caesar2020nuScenesAM} $val$. + iNet indicates that the camera encoder is pre-trained on ImageNet~\cite{deng2009imagenet} in a fully-supervised way. 
 	}
\vspace{-5mm}
	\label{tab:nuscene_det_sup_train}
\end{table}
\renewcommand{\arraystretch}{0.6}
